Safely Learning Dynamical Systems from Short Trajectories

A fundamental challenge in learning to control an unknown dynamical system is to reduce model uncertainty by making measurements while maintaining safety. In this work, we formulate a mathematical definition of what it means to safely learn a dynamical system by sequentially deciding where to initialize the next trajectory. In our framework, the state of the system is required to stay within a given safety region under the (possibly repeated) action of all dynamical systems that are consistent with the information gathered so far. For our first two results, we consider the setting of safely learning linear dynamics. We present a linear programming-based algorithm that either safely recovers the true dynamics from trajectories of length one, or certifies that safe learning is impossible. We also give an efficient semidefinite representation of the set of initial conditions whose resulting trajectories of length two are guaranteed to stay in the safety region. For our final result, we study the problem of safely learning a nonlinear dynamical system. We give a second-order cone programming based representation of the set of initial conditions that are guaranteed to remain in the safety region after one application of the system dynamics.

==> problem_formulation.tex <==
\section{Problem Formulation}
We consider a discrete-time dynamical system
\begin{equation}\label{eq:dynamics}
x_{k+1} = f(x_k),
\end{equation}
where $x\in \R^n$ is the state of the system and $f: \R^n \rightarrow \R^n$ is an unknown map that we would like to learn by making queries to the system.
% We examine a dynamical system with state variable $x \in \R^n$.
% We have a discrete time dynamics defined by a function $f: \R^n \rightarrow \R^n$.
% Thus the state evolves like so:
We consider a setting where we are given as input a set $S \subset \R^n$, called the \emph{safety region}, in which the state should remain throughout the learning process. More precisely, in order to learn $f$, we are only allowed to query points that are in $S$ and that remain in $S$ under the dynamics (\ref{eq:dynamics}) for a short time period. Obviously, if we know nothing about $f$, this task is impossible. We assume, therefore, that the dynamics $f$ belongs to a set of dynamics $U_f$, which we call the \emph{uncertainty set}. Our aim, in a sense, is to model the interplay between \emph{safety} and \emph{uncertainty} in learning dynamical systems. 



We define the \emph{safe learning problem} as the problem of learning the action of $f$ on $S$ via 


We are also interested in identifying conditions on $f$, $S$, $U_f$ under which we can safely learn $f$

the safe learning problem can be tractably solved using techniques from conic optimization.

***Motivate short time period
***Bring in out interest in classifying tractability /optimization viewpoint
*Objective function
*** One and two step safe...
*** Outline of contributions (linear 1 step 2 step, extension to nonlinear)
*** CT motivation of Vikas
***Characterizing safety region

** Define T step safety

**** Value of collecting information on the fly





Our trajectories must initiate within the safety region and should remain in the safety region under the dynamics of the system.
The (possibly repeated) action of $f$ to the point that we query should also 
We do not know the function $f$, but we may assume it belongs to a set of dynamics; i.e. $f \in U_f$.
% One special case we investigate is linear dynamics, i.e. when $f(x) = A x$ for some $A \in \R^{n \times n}$.
% Here we may assume that $A$ belongs to a set of matrices; i.e. $A \in U_A \subset \R^{n \times n}$.

We refer to points in the safety region as \emph{safe}.
The broad problem we approach in this paper is to learn the dynamics safely.
More precisely, we would like to learn $f$ in a way such that the state variable never leaves the safety region.
We can consider choosing an $x_0$ and then observing a \emph{trajectory} of length $t$, i.e. $\left \{ x_k \mid k = 1, \dots ,t \right \}$.
Each trajectory gives information on the dynamics.
Of course, to maintain safety we must ensure that $x_0$ is safe and that $x_k$ remains safe.
We say a point $x$ is \emph{one-step safe} if $x \in S$ and $f(x) \in S$.
We say a point $x$ is \emph{two-step safe} if $x \in S$ and $f(x) \in S$ and $f(f(x)) \in S$.
In certain cases, we can characterize how many trajectories we need to exactly learn the dynamics $f$.
We may also consider a cost of learning, i.e. there may be a cost to starting a trajectory at a certain point.
In this case we wish to learn the dynamics not only safely, but also with minimum cost.
